SoundCollage: Automated Discovery of New Classes in Audio Datasets

Developing new machine learning applications often requires the collection of new datasets. However, existing datasets may already contain relevant information to train models for new purposes. We propose SoundCollage: a framework to discover new classes within audio datasets by incorporating (1) an audio pre-processing pipeline to decompose different sounds in audio samples, and (2) an automated model-based annotation mechanism to identify the discovered classes. Furthermore, we introduce the clarity measure to assess the coherence of the discovered classes for better training new downstream applications. Our evaluations show that the accuracy of downstream audio classifiers within discovered class samples and a held-out dataset improves over the baseline by up to 34.7% and 4.5%, respectively. These results highlight the potential of SoundCollage in making datasets reusable by labeling with newly discovered classes. To encourage further research in this area, we open-source our code at https://github.com/nokia-bell-labs/audio-class-discovery.

==> excluded_texts/3_motivation.tex <==
\section{Motivation}
\label{motiv}

\subsection{Agreement Score Behavior for Random- and Human-labeled Tasks}

% \begin{table}[t]
% \caption{Agreement scores on human-labeled tasks from ESC-50 and SONYC-UST Engine datasets.}
% \label{tab:as_human_labeled_tasks}
% \begin{tabular}{cccrrrr}
% \hline
% \multirow{2}{*}{Task}  & \multirow{2}{*}{Model}      & \multirow{2}{*}{Dataset}                                                    & \multirow{2}{*}{Batch size} & \multicolumn{1}{c}{\multirow{2}{*}{Epoch}} & \multicolumn{2}{c}{Agreement Score}                  \\
%                        &                             &                                                                             &                             & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Stdev} \\ \hline \hline
% \multirow{14}{*}{Real} & \multirow{14}{*}{ResNet-18} & \multirow{9}{*}{ESC-50}                                                     & \multirow{3}{*}{8}          & 5                                          & 0.768                    & 0.203                     \\
%                        &                             &                                                                             &                             & 10                                         & 0.839                    & 0.164                     \\
%                        &                             &                                                                             &                             & 15                                         & 0.839                    & 0.162                     \\ \cline{4-7} 
%                        &                             &                                                                             & \multirow{3}{*}{16}         & 5                                          & 0.752                    & 0.316                     \\
%                        &                             &                                                                             &                             & 10                                         & 0.789                    & 0.190                     \\
%                        &                             &                                                                             &                             & 15                                         & 0.849                    & 0.157                     \\ \cline{4-7} 
%                        &                             &                                                                             & \multirow{3}{*}{32}         & 5                                          & 0.661                    & 0.409                     \\
%                        &                             &                                                                             &                             & 10                                         & 0.772                    & 0.308                     \\
%                        &                             &                                                                             &                             & 15                                         & 0.801                    & 0.237                     \\ \cline{3-7} 
%                        &                             & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}SONYC-UST\\ engine\end{tabular}} & \multirow{3}{*}{32}         & 10                                         & 1.000                    & 0.000                     \\
%                        &                             &                                                                             &                             & 50                                         & 1.000                    & 0.000                     \\
%                        &                             &                                                                             &                             & 100                                        & 1.000                    & 0.000                     \\ \cline{4-7} 
%                        &                             &                                                                             & \multirow{2}{*}{64}         & 50                                         & 0.997                    & 0.006                     \\
%                        &                             &                                                                             &                             & 100                                        & 1.000                    & 0.000                     \\ \hline
% \end{tabular}
% \end{table}

\begin{table*}[t]
\centering
\caption{Agreement scores on human- and random-labeled tasks from AudioSet Speech dataset.}
\label{tab:as_human_labeled}
\begin{tabular}{clcccrr}
\hline
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Task}}}                      & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Batch size}} & \multirow{2}{*}{\textbf{Epoch}} & \multicolumn{2}{c}{\textbf{Agreement Score}}                         \\ \cline{6-7} 
\multicolumn{2}{c}{}                                                    &                                 &                                      &                                 & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{Std}} \\ \hline \hline
\multirow{4}{*}{Real} & Babbling                      & \multirow{5}{*}{ResNet-18}      & \multirow{5}{*}{8}                   & \multirow{10}{*}{50}            & 0.940506                                 & 0.0310349                               \\ \cline{2-2}
                               & Female speech, woman speaking &                                 &                                      &                                 & 0.83544305                                 & 0.077572886                                \\ \cline{2-2}
                               & Male speech, man speaking     &                                 &                                      &                                 & 0.888607609                                 & 0.028492738                                \\ \cline{2-2}
                               & Child speech, kid speaking    &                                 &                                      &                                 & 0.745569646                                 & 0.05217415                                \\ \cline{1-2} \cline{6-7} 
\multicolumn{2}{c}{Random}                                     &                                 &                                      &                                 & 0.588607609                                 & 0.07066723                                \\ \cline{1-4} \cline{6-7} 
\multirow{4}{*}{Real} & Babbling                      & \multirow{5}{*}{ResNet-18}      & \multirow{5}{*}{16}                  &                                 & 0.943038                          & 0.02478342                       \\ \cline{2-2}
                               & Female speech, woman speaking &                                 &                                      &                                 & 0.754430                          & 0.17005842                       \\ \cline{2-2}
                               & Male speech, man speaking     &                                 &                                      &                                 & 0.826582                                 & 0.12474760                                \\ \cline{2-2}
                               & Child speech, kid speaking    &                                 &                                      &                                 & 0.773417741                                 & 0.036516789                                \\ \cline{1-2} \cline{6-7} 
\multicolumn{2}{c}{Random}                                     &                                 &                                      &                                 & 0.588607615                                & 0.065434869                                \\ \hline
\end{tabular}

\end{table*}

% AS differentiates human- from random-labeled tasks
We investigated the validity of the given agreement score (AS) for discriminating practical tasks in audio data (i.e.,~ESC-50, SONYC-UST and AudioSet datasets). Tables~\ref{tab:as_human_labeled_tasks} and ~\ref{tab:as_human_labeled} outlines the agreement scores for human- and random-labeled tasks. \hr{Need experiments with random-labeled ESC-50 and SONYC-UST datasets.} The empirical distribution of AS for randomly labeled tasks is generally below~0.6, whereas for human-labeled tasks, it consistently exceeds~0.7. Based on these results, we can conclude that AS could serve as a useful cue for determining practical audio tasks from machine learning model's perspective.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/task_viz_speech_baseline.pdf}
%     \caption{Visualization of discovered tasks by baseline.}
%     \label{fig:task_viz_speech_baseline}
% \end{figure}

However, this does not imply that AS alone can serve as a cue to determine meaningful audio tasks from a human's perspective. We investigated whether humans could comprehend the meaning of discovered tasks solely by relying on AS. Figure~\ref{fig:task_viz_speech_baseline} illustrates mel-spectrograms of twenty representative samples for each class within each discovered task. Identifying patterns in these samples proves to be extremely challenging. This challenge aligns with observations from a prior study focused on discovering potential image-based tasks~\cite{}. Consequently, it is difficult to assert that the tasks discovered by AS are interpretable through visual inspection. This challenge may stem from the fact that the samples are audio samples, not visual ones. To address this, we attempted to interpret the meaning of classes for each task by obtaining predictions from a large audio classification model, YAMNet.


We selected the top 20 representative samples for each class.\footnote{Each task is a binary classification task, resulting in two distinct classes.} Subsequently, we obtained the top 10 high probability predictions for each sample from YAMNet. Following this, for each identified label from YAMNet prediction results, we calculated the proportion of samples with that label. We then extracted tasks only in which a proportion gap larger than 0.5 exists between the two classes. Table~\ref{tab:valid_tasks_baseline} provides details on the extracted tasks where such a gap in the proportion of samples with the corresponding label exceeds 0.5.


While we managed to extract a few tasks with lenient criteria, we could not identify classes that are clearly discriminable by audio. \hr{Need a reasonable criteria to determine PRACTICAL audio tasks. Can we come up with a straightforward yet robust method to add on top of YAMNet?} Furthermore, we did not observe any correlation between interpretability by audio and agreement score. \hr{Is it feasible to devise a metric that correlates with the practicality of discovered tasks?} In response to these observations, we attempted to propose an advanced framework for discovering potential tasks that are interpretable by humans within the context of audio datasets.


% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_8_5.png}
%          \caption{epoch=5}
%          \label{fig:esc50_resnet_8_5}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_8_10.png}
%          \caption{epoch=10}
%          \label{fig:esc50_resnet_8_10}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_8_15.png}
%          \caption{epoch=15}
%          \label{fig:esc50_resnet_8_15}
%      \end{subfigure}
%         \caption{Distribution and trend of agreement scores of human-labled tasks in ESC-50 (batch\_size=8).}
%         \label{fig:esc50_8}
% \end{figure}
% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_16_5.png}
%          \caption{epoch=5}
%          \label{fig:esc50_resnet_16_5}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_16_10.png}
%          \caption{epoch=10}
%          \label{fig:esc50_resnet_16_10}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_16_15.png}
%          \caption{epoch=15}
%          \label{fig:esc50_resnet_16_15}
%      \end{subfigure}
%         \caption{Distribution and trend of agreement scores of human-labled tasks in ESC-50 (batch\_size=16).}
%         \label{fig:esc50_16}
% \end{figure}
% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_32_5.png}
%          \caption{epoch=5}
%          \label{fig:esc50_resnet_32_5}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_32_10.png}
%          \caption{epoch=10}
%          \label{fig:esc50_resnet_32_10}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures_res/resnet_32_15.png}
%          \caption{epoch=15}
%          \label{fig:esc50_resnet_32_15}
%      \end{subfigure}
%         \caption{Distribution and trend of agreement scores of human-labled tasks in ESC-50 (batch\_size=32).}
%         \label{fig:esc50_32}
% \end{figure}




==> excluded_texts/4_methodology.tex <==


\begin{comment}
%--Step-by-step explanation--%
\subsection{Step 1: Train multiple encoders}
\label{method:step1}

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\textwidth]{figures/method_step1.png}
    \caption{$x_{train}$: Public datasets with the same modalities and different collection objectives. $f_n(x)$: Output of a signal processing technique. $v_x^n$: Feature vector output from an encoder. $y_x^n$: Reconstruction from a decoder.}
    \label{fig:method_step1}
\end{figure}

\textbf{Context.} Different efficient signal processing methods for different tasks.

\textbf{Intuition.} When we input the features processed by each signal processing technique into the encoder, the encoder generates embeddings based on those features, and we perform clustering on these embeddings, we may be able to investigate whether the clustering results align with suitable tasks corresponding to each signal processing method.

\textbf{Approach.} Training multiple encoders, clustering feature embeddings, and matching them with corresponding labels.

\textbf{Assumption.} We possess a limited labeled dataset specifically tailored to our task and aim to leverage additional publicly available datasets to enhance our task.

Train separate encoders, where each encoder takes as input the processed signal obtained using a different signal processing method. The goal is to capture the distinctive features or representations specific to each signal-processing technique. By training these encoders separately, we create distinct feature embeddings for each signal processing method.

\subsection{Step 2: Clustering of feature embeddings}
\label{method:step2}

\begin{figure}[t]
    \begin{subfigure}{0.4\textwidth}
    \raggedleft
    \includegraphics[width=\textwidth]{figures/method_step2_xtest.png}
    \caption{$x_{test}$: A public dataset we want to check if the dataset can be utilized for our task.}
    \end{subfigure}
    \begin{subfigure}{0.51\textwidth}
    \includegraphics[width=\textwidth]{figures/method_step2_xours.png}
    \caption{$x_{ours}$: Limited dataset collected for our task.}
    \raggedright
    \end{subfigure}
\end{figure}

Apply clustering algorithms to the feature embeddings obtained from each encoder. The clustering algorithm will group similar feature representations together, creating clusters that may correspond to different underlying tasks. This step aims to identify patterns or similarities in the extracted features.


\subsection{Step 3: Task-label matching}
\label{method:step3}

\begin{figure}[t]
    \begin{subfigure}{0.485\textwidth}
    \raggedleft
    \includegraphics[width=\textwidth]{figures/method_step3.png}
    \caption{}
    \label{fig:method_step3}
    \end{subfigure}
    \begin{subfigure}{0.485\textwidth}
    \includegraphics[width=\textwidth]{figures/method_step3_corr.png}
    \caption{}
    \label{fig:method_step3_corr}
    \raggedright
    \end{subfigure}
\end{figure}

Once the clusters are formed, compare them with the available labels of corresponding tasks. The assumption is that if the features from a particular signal processing method are meaningful to a certain task, the resulting clusters would align well with the labels associated with that task. By analyzing the correspondence between clusters and labels, we can infer the potential tasks supported by the different signal-processing methods.

\noindent Q. Can we utilize the test dataset for our task?
Assess the similarities between the distributions of feature embeddings from two distinct datasets, $x_{test}$ and $x_{ours}$.

\noindent Q. Can we find general correlations between labels from different tasks?
Investigate correlations between the labels in the test dataset ($x_{test}$) and the labels in our dataset ($x_{ours}$) (Fig.~\ref{fig:method_step3_corr}).
\end{comment}

==> excluded_texts/6_evaluation.tex <==

\begin{table}[ht]
\begin{tabular}{llll}
\hline
\textbf{Baseline} & \textbf{domestic\_sounds\_home\_sounds}    &                  &             \\ \hline
\textbf{Task ID}  & \textbf{Label from Pre-trained Classifier} & \textbf{Clarity} & \textbf{AS} \\ \hline\hline
21                & Glockenspiel                               & 0.95             & 0.90279466  \\
14                & Bowed string instrument                    & 0.75             & 0.91373026  \\
22                & Child speech, kid speaking                 & 0.55             & 0.92588091  \\
27                & Silence                                    & 0.55             & 0.9052248   \\
23                & Fill (with liquid)                         & 0.45             & 0.91251516  \\ \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\begin{tabular}{llll}
\hline
\textbf{Baseline} & \multicolumn{2}{l}{\textbf{outside\_urban\_or\_manmade}}      &             \\ \hline
\textbf{Task ID}  & \textbf{Label from Pre-trained Classifier} & \textbf{Clarity} & \textbf{AS} \\ \hline\hline
0                 & Boat, Water vehicle                        & 0.75             & 0.88663524  \\
27                & Bus                                        & 0.7              & 0.86604726  \\
5                 & Inside, large room or hall                 & 0.6              & 0.90464973  \\
8                 & Tools                                      & 0.6              & 0.91995984  \\
6                 & Tools                                      & 0.5              & 0.8825351   \\ \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\begin{tabular}{llll}
\hline
\textbf{Ours}    & \multicolumn{2}{l}{\textbf{domestic\_sounds\_home\_sounds\_fore}} &             \\ \hline
\textbf{Task ID} & \textbf{Label from Pre-trained Classifier}   & \textbf{Clarity}   & \textbf{AS} \\ \hline\hline
4                & Violin, fiddle                               & 0.7                & 0.93206668  \\
25               & Bowed string instrument                      & 0.55               & 0.90802634  \\
16               & Violin, fiddle                               & 0.45               & 0.9202016   \\
22               & Animal                                       & 0.45               & 0.93819308  \\
24               & Theme music                                  & 0.45               & 0.86622721  \\ \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\begin{tabular}{llll}
\hline
\textbf{Ours}    & \multicolumn{2}{l}{\textbf{domestic\_sounds\_home\_sounds\_back}} &             \\ \hline
\textbf{Task ID} & \textbf{Label from Pre-trained Classifier}   & \textbf{Clarity}   & \textbf{AS} \\ \hline\hline
27               & Cello                                        & 0.95               & 0.87008035  \\
6                & Engine                                       & 0.65               & 0.92258376  \\
13               & Silence                                      & 0.6                & 0.90992451  \\
26               & Wood                                         & 0.6                & 0.92169112  \\
4                & Gong                                         & 0.5                & 0.86277694  \\ \hline
\end{tabular}
\end{table}



\begin{table}[ht]
\caption{Valid discovered tasks from the baseline. Valid tasks are identified based on the presence of a gap exceeding 0.5 in the proportion of samples with an identical label between two classes within each discovered task.}
\label{tab:valid_tasks_baseline}
\begin{tabular}{cclcc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task ID}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{AS}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Label from YAMNet}}} & \multicolumn{2}{c}{\textbf{Proportion of Samples}}                          \\ \cline{4-5} 
\multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{}                             & \multicolumn{1}{c}{}                                            & \multicolumn{1}{c}{\textbf{Class 0}} & \multicolumn{1}{c}{\textbf{Class 1}} \\ \hline\hline
1                                                     & 0.85                                             & Snake                                                           & 0.10                                 & 0.60                                 \\
2                                                     & 0.82                                             & Breathing                                                       & 0.90                                 & 0.25                                 \\
2                                                     & 0.82                                             & Snoring                                                         & 0.70                                 & 0.15                                 \\
19                                                    & 0.84                                             & Musical instrument                                              & 0.20                                 & 0.70                                 \\
25                                                    & 0.73                                             & Motor vehicle (road)                                            & 0.05                                 & 0.55                                 \\
25                                                    & 0.73                                             & Car                                                             & 0.05                                 & 0.55                                 \\
26                                                    & 0.82                                             & Singing                                                         & 0.10                                 & 0.60                                 \\ \hline
\end{tabular}
\end{table}
\begin{table}[ht]
\caption{Valid discovered tasks from DITTO. Valid tasks are identified based on the presence of a gap existing 0.5 in the proportion of samples with an identical label between two classes within each discovered task.}
\label{tab:valid_tasks_ditto}
\begin{tabular}{cclcc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task ID}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{AS}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Label from YAMNet}}} & \multicolumn{2}{c}{\textbf{Proportion of Samples}}                          \\ \cline{4-5} 
\multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{}                             & \multicolumn{1}{c}{}                                            & \multicolumn{1}{c}{\textbf{Class 0}} & \multicolumn{1}{c}{\textbf{Class 1}} \\ \hline
4                                                     & 0.96                                             & Silence                                                         & 0.15                                 & 0.85                                 \\
4                                                     & 0.96                                             & Music                                                           & 0.00                                 & 0.60                                 \\
6                                                     & 0.92                                             & Child speech, kid speaking                                      & 0.05                                 & 0.55                                 \\
6                                                     & 0.92                                             & Child singing                                                   & 0.00                                 & 0.60                                 \\
9                                                     & 0.91                                             & Speech                                                          & 0.90                                 & 0.35                                 \\
9                                                     & 0.91                                             & Child speech, kid speaking                                      & 0.55                                 & 0.05                                 \\
17                                                    & 0.91                                             & Silence                                                         & 0.35                                 & 0.90                                 \\
20                                                    & 0.93                                             & Singing                                                         & 0.00                                 & 0.70                                 \\
22                                                    & 0.94                                             & Conversation                                                    & 0.60                                 & 0.10                                 \\
23                                                    & 0.95                                             & Silence                                                         & 0.05                                 & 0.60                                 \\
27                                                    & 0.91                                             & Singing                                                         & 0.00                                 & 0.55                                 \\
29                                                    & 0.94                                             & Music                                                           & 0.00                                 & 0.75                                 \\
31                                                    & 0.94                                             & Inside, small room                                              & 0.30                                 & 0.95                                 \\
31                                                    & 0.94                                             & Silence                                                         & 0.00                                 & 0.65                                 \\ \hline
\end{tabular}
\end{table}


==> sections/author_response.tex <==
\section*{Author Response}
  We really appreciate the reviewers' insightful feedback. We have grouped the reviewers' comments by similar discussion points and provided a single, unified response for each group.

  \textbf{1. Using YAMNet Directly after Pre-processing (R7):} Respectfully, we believe that the reviewer may have confused our proposed approach with traditional audio classification methods and thus have misinterpreted some of the key results. The main purpose of our \system{} is to identify clear class boundaries in  the subsets of the large-scale dataset under exploration that might correspond to some meaningful classes. Thus, \system{} does not aim to compete with audio classification models (e.g., YAMNet) in predicting the label. Instead, \system{} aim to search within the dataset for subsets of samples that can provide a dataset for a given task that provide a more generalizable class boundary than just randomly labeling some samples. This, in turn, would allow us to use the discovered subset to better train new models with the desired task. Considering this, the ``classification accuracy'' is not the right metric for comparison of our work, instead the main purpose is to evaluate how well \system{} has discovered a generalizable class boundary, which for this purpose we utilize \textit{agreement scores} and our proposed \textit{clarity}. 
% Therefore, we use YAMNet in this work to label the classes only after observing the key class boundaries present in the dataset and reduce human effort.

\textbf{2. Clarifying the \textit{Clarity} Metric (R6, R7):}
The \textit{clarity} is introduced to evaluate how distinctive two classes are when concerning a specified task. Thus, in principle, the purpose of \textit{clarity} metric is different from conventional classification accuracy as a metric. To prioritize the identification of a clear class boundary, rather than simply predicting a class label, a higher \textit{clarity} indicates that the samples are more distinctly separated in the state space, which results in a larger number of samples that accurately represent their discovered class. In the example provided in the Section~\ref{sec:clarity}%on ``Page 3''
, we show that for task $\tau_1$, there is a less clear boundary as some of the samples with label $Y_0$ are present in both sides of the decision boundary. Conversely, task $\tau_2$ offers a more precise class boundary as there are no samples in the wrong side, thus offering a higher quality (i.e., less noisy) training set for the downstream task. 

  \textbf{3. Clarification on The Input Data Shape (R6, R7, R8):}
We acknowledge the confusion regarding the input data shape caused by unclear wording in the Section III.B. To clarify, we processed input data for both the baseline and \system{} after the signal pre-processing pipeline as follows: (i) For the baseline, we used raw audio samples, all 10 seconds in length. (ii) For \system{}, we used pre-processed audio samples, which were either equal to or shorter than 10 seconds. (iii) For both baseline and \system{} the data were standardized into a fixed 64x64 MFCC representation, corresponding to 10-second audio segments. (iv) For samples shorter than 10 seconds, we applied zero-padding to extend them to the target length. Using a 25ms window with a 10ms overlap, we extracted 64 mel frequency bands and calculated MFCCs, yielding approximately 1000 frames for a 10-second clip. (v) All the frames were then resampled to 64 time steps using linear interpolation, ensuring consistent temporal resolution across all samples.

  \textbf{4.The need for evaluation with human annotators (R6, R7, R8):}
We acknowledge the potential value of involving large-scale and well-established human annotators to assess the discovered classes and their differences from automated annotations (R6, R7) as well as verifying the accuracy of the discovered labels (R8). However, the unlimited label space poses significant challenges and costs in conducting experiments with human annotators. For instance, YAMNet evaluates the probabilities of 521 labels for each sample, and we use the clarity metric to assess the class annotations. We would like to emphasize that requesting human annotators to evaluate audio samples across such a large or unlimited label space for every instance is impractical and would be extremely costly. Nonetheless, we believe that future work could benefit from an extended and more comprehensive approach, incorporating focused evaluations with human annotators to provide deeper insights and inform further enhancements to \system{}.

  \textbf{7. Ablation Studies (R7):} We would like to point that ablation studies of our paper are present in all the key results \figurename~\ref{fig:main_perf}, \tablename~\ref{tab:clarity}, \tablename~\ref{tbl:diversity}, \tablename~\ref{tab:downstream_cross}, and \tablename~\ref{tab:downstream}.
These baseline comparisons serve as the ablation study as we remove the necessary pre-processing steps and adaptations to the task discovery framework for them. 

  \textbf{8. No Correlation between AS and Clarity is not Intuitive (R7):} The \textit{agreement score} (AS) measures the similarity between two randomly initialized neural networks (\cite{atanov2022task} of the main draft) whereas the clarity metric measures how distinct two classes are concerning a particular class boundary. In principle, each of these metrics evaluate our \system{} from different perspectives: one from the ability to generalize the class boundary (using \textit{agreement scores}) and distinctiveness of the discovered class boundaries (using \textit{clarity} metric).

  \textbf{9. Incomplete References (R6):} We will address inaccuracies in our references, however, we would like to emphasize that citing papers available exclusively on arXiv (or those previously rejected) is a common practice in the  community. Such works often represent recent advancements and provide valuable information worthy of citation. We included these references for their relevance and will ensure to locate and cite the most recent version of each paper. 

  \textbf{10. Modeling Performance on the Original Set (R3):} Although this is an interesting suggestion, it is extremely challenging to perform this as there might not be benchmark datasets available for all the discovered classes. However, in \tablename~\ref{tab:downstream_cross} of the our paper we perform a cross-validation on the same dataset to assess the quality of the labeled dataset. 

  \textbf{11. Threshold for Class Discovery (R6):} The threshold for discovering new classes is a configurable design parameter. Setting it closer to 1 favors the identification of fewer, well-separated classes, while setting it closer to 0.5 promotes the discovery of more classes that may be less distinct.

  \textbf{12. Does not Inform about the Labeling Accuracy (R8):} As the main objective of our paper is to find hidden classes in real-world audio datasets, we had no access to any existing ground-truth labels due to which we cannot find label accuracy. Additionally, instead of label accuracy we assess the quality of the discovered classes using \textit{clarity}, a metric defined by us in the main draft Eqn.~\ref{eqn:clarity} of the main draft.

  Finally, regarding other suggestions from all the reviewers (on \textbf{tone adjustment and language changes)}, we agree that our claims, methodology, and results can be presented more effectively, and we will revise them accordingly. Additionally, we will ensure that the final draft is thoroughly proofread and free of errors.
